SyReNets: Symbolic Residual Neural Networks

Despite successful seminal works on passive systems in the literature, learning free-form physical laws for controlled dynamical systems given experimental data is still an open problem. For decades, symbolic mathematical equations and system identification were the golden standards. Unfortunately, a set of assumptions about the properties of the underlying system is required, which makes the model very rigid and unable to adapt to unforeseen changes in the physical system. Neural networks, on the other hand, are known universal function approximators but are prone to over-fit, limited accuracy, and bias problems, which makes them alone unreliable candidates for such tasks. In this paper, we propose SyReNets, an approach that leverages neural networks for learning symbolic relations to accurately describe dynamic physical systems from data. It explores a sequence of symbolic layers that build, in a residual manner, mathematical relations that describes a given desired output from input variables. We apply it to learn the symbolic equation that describes the Lagrangian of a given physical system. We do this by only observing random samples of position, velocity, and acceleration as input and torque as output. Therefore, using the Lagrangian as a latent representation from which we derive torque using the Euler-Lagrange equations. The approach is evaluated using a simulated controlled double pendulum and compared with neural networks, genetic programming, and traditional system identification. The results demonstrate that, compared to neural networks and genetic programming, SyReNets converges to representations that are more accurate and precise throughout the state space. Despite having slower convergence than traditional system identification, similar to neural networks, the approach remains flexible enough to adapt to an unforeseen change in the physical system structure.

==> Symbolic Residual Neural Networks/tex/comment.tex <==
% define simple todo command
\usepackage[normalem]{ulem}                                        % <- for striking text out
\usepackage{marginnote}
\setlength{\marginparwidth}{1.5cm}
\usepackage[textwidth=10ex,colorinlistoftodos]{todonotes}
\newcommand{\tinytodo}[2][]
{\todo[caption={#2}, size=\footnotesize, #1]{\renewcommand{\baselinestretch}{0.5}\selectfont#2\par}}
\providecommand{\usage}{\input{tex/usage}}
% define colours for to-dos
\colorlet{jb}{red}
\colorlet{fw}{red}
\colorlet{cv}{green}
\colorlet{sh}{blue}

\newcommand  {\note}[1]{{\color{gray}#1}}
\newcommand  {\done}[1]{\sout{#1}}
\newcommand  {\jb}  [1]{\tinytodo[color=white,nolist,linecolor=jb,bordercolor=white,noinline]{\protect{\scriptsize\color{jb}#1}}}
\newcommand  {\fw}  [1]{\tinytodo[color=white,linecolor=fw,bordercolor=white,noinline]{\protect{\footnotesize\color{fw}#1}}}
\newcommand  {\cv}  [1]{\tinytodo[color=white,linecolor=cv,bordercolor=white,noinline]{\protect{\footnotesize\color{cv}#1}}}
\newcommand  {\sh}  [1]{\tinytodo[color=white,linecolor=sh,bordercolor=white,noinline]{\protect{\footnotesize\color{sh}#1}}}
% comment above, and uncomment below to remove todo list.
%\usepackage[disable]{todonotes}\renewcommand{\usage}{}%\newcommand{\mh}[3]{#3}{}{}\newcommand{\maybedo}[1]{}

\newcommand{\atCV} {{\color{cv}@CV}}
\newcommand{\atFW} {{\color{fw}@FW}}
\newcommand{\atSH} {{\color{sh}@SH}}
\newcommand{\atALL}{\atCV, \atFW, \atSH}

\newcommand{\commentcolourcode}{Comments colour code: 
{\color{cv}CV}, 
{\color{fw}FW}, 
{\color{sh}SH}} 

\providecommand{\edit}[2]{\sout{#1}~{\color{change}#2}}
\renewcommand{\sout}[1]{}
\colorlet{change}{blue}

==> Symbolic Residual Neural Networks/tex/format.tex <==

% define format of some common idioms
\newcommand{\eg}{\textit{e.g.,}~} %
\newcommand{\ie}{\textit{i.e.,}~} %
\newcommand{\ca}{\textit{ca.}~}   %
\newcommand{\qv}{\textit{q.v.,}~} %
\newcommand{\cf}{\textit{cf.}~} %
\newcommand{\apriori}{\textit{a~priori}} %
\newcommand{\etc}{\textit{etc.}}  %
\newcommand{\naive}{na\"ive}      %
\newcommand{\etal}{\textit{et al.}~} %


==> Symbolic Residual Neural Networks/tex/preamble.tex <==

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors

\usepackage{textcomp}     % access \textquotesingle
% \vspace{-10pt}


\input{tex/format}
% \input{tex/comment}

==> Symbolic Residual Neural Networks/tex/usage.tex <==
\section*{Usage notes}~\\%[1ex]
%\paragraph*{Comments}~\\%[1ex]
\noindent Use \texttt{\textbackslash yourinitials\{your comment\}} to add comments/to dos. For example,
\underline{J}oe \underline{B}loggs adds comments using \texttt{\textbackslash jb\{Comment.\}}.\jb{These comments will appear as margin notes. They will also appear in the todo list on the first page.} \\[2ex]
\noindent Use \texttt{\textbackslash atInitials} to address your comment to someone (\eg \texttt{\textbackslash jb\{\textbackslash atMH: Please fix this.\}}).\\[2ex]
You can mark a comment as resolved using \texttt{\textbackslash done\{Comment text.\}}, (\eg \texttt{\textbackslash jb\{\textbackslash done\{\textbackslash atMH: Please fix this.\}\}}). It will then be formatted like this: \done{\atMH: Please fix this.}.\\[2ex]
\commentcolourcode\\[1ex]
%\noindent\note{Guidance text from the call is formatted like this.}\\[2ex]
%\paragraph*{Work packages/tasks/deliverables, referencing}~\\%[1ex]
%\emph{Work package descriptions} are added as:\\[1ex]
%\texttt{\textbackslash work package\{wp\_label\}\{Work package title\}\{Lead partner\}\{start\_month\}\{end\_month\}\{\\
%Objectives description text.\\
%\}\\
%\{\\
%Task descriptions.\\
%\}\\
%\{\\
%Deliverables descriptions.\\
%\}\\
%}\\[1ex]
%To refer to work packages in the text, you can use:\\[1ex]
%\texttt{\textbackslash wpref\{wp\_label\}} (will format the reference as `WPX'), or \\
%\texttt{\textbackslash ref\{wp:wp\_label\}} (will just give the WP number, \ie `X').\\[2ex]
%%
%To add \emph{task descriptions} you can use:\\[1ex]
%\texttt{\textbackslash task\{task\_label\}\{Task title\}\{List of partners (lead partner in \textbf{bold})\}\{start\_month\}\{end\_month\}\{\\
%Task description text.\}}\\[1ex]
%To refer to that task in the text, you can use:\\[1ex]
%\texttt{\textbackslash tkref\{task\_label\}} (will format the reference as `TX.X'), or \\
%\texttt{\textbackslash ref\{tk:task\_label\}} (will just give the number, \ie `X.X').\\[2ex]
%%
%To add \emph{deliverables descriptions} you can use:\\[1ex]
%\texttt{\textbackslash deliverable\{deliverable\_label\}\{Deliverable description text\}\{Partner(s) responsible\}\{month\_due\}\{deliverable\_type\}\{dissemination\_level\}}\\[1ex]
%To refer to it in the text, you can use:\\[1ex]
%\texttt{\textbackslash dref\{deliverable\_label\}} (will format the reference as `DX.X'), or \\
%\texttt{\textbackslash ref\{d:deliverable\_label\}} (will just give the number, \ie `X.X').\\[2ex]

\listoftodos~\\[2ex]

\clearpage\setcounter{page}{1}




==> tex/comment.tex <==
% define simple todo command
\usepackage[normalem]{ulem}                                        % <- for striking text out
\usepackage{marginnote}
\setlength{\marginparwidth}{1.5cm}
\usepackage[textwidth=10ex,colorinlistoftodos]{todonotes}
\newcommand{\tinytodo}[2][]
{\todo[caption={#2}, size=\footnotesize, #1]{\renewcommand{\baselinestretch}{0.5}\selectfont#2\par}}
\providecommand{\usage}{\input{tex/usage}}
% define colours for to-dos
\colorlet{jb}{red}
\colorlet{fw}{red}
\colorlet{cv}{green}
\colorlet{sh}{blue}

\newcommand  {\note}[1]{{\color{gray}#1}}
\newcommand  {\done}[1]{\sout{#1}}
\newcommand  {\jb}  [1]{\tinytodo[color=white,nolist,linecolor=jb,bordercolor=white,noinline]{\protect{\scriptsize\color{jb}#1}}}
\newcommand  {\fw}  [1]{\tinytodo[color=white,linecolor=fw,bordercolor=white,noinline]{\protect{\footnotesize\color{fw}#1}}}
\newcommand  {\cv}  [1]{\tinytodo[color=white,linecolor=cv,bordercolor=white,noinline]{\protect{\footnotesize\color{cv}#1}}}
\newcommand  {\sh}  [1]{\tinytodo[color=white,linecolor=sh,bordercolor=white,noinline]{\protect{\footnotesize\color{sh}#1}}}
% comment above, and uncomment below to remove todo list.
%\usepackage[disable]{todonotes}\renewcommand{\usage}{}%\newcommand{\mh}[3]{#3}{}{}\newcommand{\maybedo}[1]{}

\newcommand{\atCV} {{\color{cv}@CV}}
\newcommand{\atFW} {{\color{fw}@FW}}
\newcommand{\atSH} {{\color{sh}@SH}}
\newcommand{\atALL}{\atCV, \atFW, \atSH}

\newcommand{\commentcolourcode}{Comments colour code: 
{\color{cv}CV}, 
{\color{fw}FW}, 
{\color{sh}SH}} 

\providecommand{\edit}[2]{\sout{#1}~{\color{change}#2}}
\renewcommand{\sout}[1]{}
\colorlet{change}{blue}

==> tex/usage.tex <==
\section*{Usage notes}~\\%[1ex]
%\paragraph*{Comments}~\\%[1ex]
\noindent Use \texttt{\textbackslash yourinitials\{your comment\}} to add comments/to dos. For example,
\underline{J}oe \underline{B}loggs adds comments using \texttt{\textbackslash jb\{Comment.\}}.\jb{These comments will appear as margin notes. They will also appear in the todo list on the first page.} \\[2ex]
\noindent Use \texttt{\textbackslash atInitials} to address your comment to someone (\eg \texttt{\textbackslash jb\{\textbackslash atMH: Please fix this.\}}).\\[2ex]
You can mark a comment as resolved using \texttt{\textbackslash done\{Comment text.\}}, (\eg \texttt{\textbackslash jb\{\textbackslash done\{\textbackslash atMH: Please fix this.\}\}}). It will then be formatted like this: \done{\atMH: Please fix this.}.\\[2ex]
\commentcolourcode\\[1ex]
%\noindent\note{Guidance text from the call is formatted like this.}\\[2ex]
%\paragraph*{Work packages/tasks/deliverables, referencing}~\\%[1ex]
%\emph{Work package descriptions} are added as:\\[1ex]
%\texttt{\textbackslash work package\{wp\_label\}\{Work package title\}\{Lead partner\}\{start\_month\}\{end\_month\}\{\\
%Objectives description text.\\
%\}\\
%\{\\
%Task descriptions.\\
%\}\\
%\{\\
%Deliverables descriptions.\\
%\}\\
%}\\[1ex]
%To refer to work packages in the text, you can use:\\[1ex]
%\texttt{\textbackslash wpref\{wp\_label\}} (will format the reference as `WPX'), or \\
%\texttt{\textbackslash ref\{wp:wp\_label\}} (will just give the WP number, \ie `X').\\[2ex]
%%
%To add \emph{task descriptions} you can use:\\[1ex]
%\texttt{\textbackslash task\{task\_label\}\{Task title\}\{List of partners (lead partner in \textbf{bold})\}\{start\_month\}\{end\_month\}\{\\
%Task description text.\}}\\[1ex]
%To refer to that task in the text, you can use:\\[1ex]
%\texttt{\textbackslash tkref\{task\_label\}} (will format the reference as `TX.X'), or \\
%\texttt{\textbackslash ref\{tk:task\_label\}} (will just give the number, \ie `X.X').\\[2ex]
%%
%To add \emph{deliverables descriptions} you can use:\\[1ex]
%\texttt{\textbackslash deliverable\{deliverable\_label\}\{Deliverable description text\}\{Partner(s) responsible\}\{month\_due\}\{deliverable\_type\}\{dissemination\_level\}}\\[1ex]
%To refer to it in the text, you can use:\\[1ex]
%\texttt{\textbackslash dref\{deliverable\_label\}} (will format the reference as `DX.X'), or \\
%\texttt{\textbackslash ref\{d:deliverable\_label\}} (will just give the number, \ie `X.X').\\[2ex]

\listoftodos~\\[2ex]

\clearpage\setcounter{page}{1}



